Resonance for life: Metabolism and Social Interactions in Bacterial Communities

The social organization of microorganisms has long been a fascinating and challenging subject in both biology and sociology. In these organisms, the role of the individual is far less dominant than that of the community, which functions as a superorganism. The coordination is achieved through a communication mechanism known as quorum sensing. When the community is healthy, quorum sensing enables it to regulate the development of potentially harmful individuals. This study employs an agent-based quorum sensing model to explore the relationship between metabolic functions and social behavior. It also examines how a polyculture responds to variations in the metabolic characteristics of its components. Finally, we identify a particularly stable condition in which the components cooperate to maximize the overall health of the colony. We refer to this state as resonance for life.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
